DataX: A system for Data eXchange and transformation of streams

The exponential growth in smart sensors and rapid progress in 5G networks is creating a world awash with data streams. However, a key barrier to building performant multi-sensor, distributed stream processing applications is high programming complexity. We propose DataX, a novel platform that improves programmer productivity by enabling easy exchange, transformations, and fusion of data streams. DataX abstraction simplifies the application's specification and exposes parallelism and dependencies among the application functions (microservices). DataX runtime automatically sets up appropriate data communication mechanisms, enables effortless reuse of microservices and data streams across applications, and leverages serverless computing to transform, fuse, and auto-scale microservices. DataX makes it easy to write, deploy and reliably operate distributed applications at scale. Synthesizing these capabilities into a single platform is substantially more transformative than any available stream processing system.

==> components.tex <==
\begin{tikzpicture}[node distance=0.6cm, auto, thick,scale=1, every node/.style={scale=0.75}]
        

    \begin{scope}[node distance=0.2cm]
        \node (driverscript) [rectangle, draw=black] {Script};
        \node (sdk) [rectangle, fill=yellow, below = of driverscript, draw] {SKD};
        \node (dric) [draw,dotted, inner sep=0.3cm, fit=(driverscript) (sdk)] {};
        \node (driversidecar) [rectangle, yshift=0.45cm, fill=yellow, right = of driverscript, minimum height=1.6cm, draw, anchor=north, xshift=0.8cm] 
{Sidecar};
        \node (driver)[draw, inner sep=0.5cm, fit=(dric) (driversidecar)] {};
    \end{scope}

    \node (sensor) [sensor, left = of driverscript] {Sensor};

    \begin{scope}[node distance=0.2cm]
        \node (auscript) [rectangle, draw=black, right = of driver, yshift=0.355cm, xshift=1cm] {Script};
        \node (ausdk) [rectangle, fill=yellow, below = of auscript,draw] {SKD};
        \node (auc) [draw,dotted, inner sep=0.3cm, fit=(auscript) (ausdk)] {};
        \node (ausidecar) [rectangle, yshift=0.45cm, fill=yellow, right = of auscript, minimum height=1.6cm, draw, anchor=north, xshift=0.8cm] {Sidecar};
        \node (au)[draw, inner sep=0.5cm, fit=(auc) (ausidecar)] {};
    \end{scope}

    \begin{scope}[node distance=0.2cm]
        \node (actsidecar) [rectangle, fill=yellow, right = of au, minimum height=1.6cm, draw, xshift=1cm] {Sidecar};
        \node (actscript) [rectangle, draw=black, right = of actsidecar, yshift=0.355cm] {Script};
        \node (actsdk) [rectangle, fill=yellow, below = of actscript,draw] {SKD};
        \node (actc) [draw,dotted, inner sep=0.3cm, fit=(actscript) (actsdk)] {};
        \node (act)[draw, inner sep=0.5cm, fit=(actc) (actsidecar)] {};
    \end{scope}

    \node (gadget) [gadget, right of = actscript, xshift=2cm] {Gadget};

    %\node (operator) [rectangle, fill=yellow, below = of sensor, xshift=10cm, minimum width=10cm] {DataX Operator};

    \node (operator) [rectangle, below = of sensor.east, anchor=west, draw=black, fill=yellow,  minimum width = 11.5cm, xshift=0.6cm, yshift=-2cm, minimum height=0.7cm] {Operator};

    \node (bus) [rectangle, above = of driver.west, anchor=west, draw=black, fill=yellow, minimum width = 11.7cm, yshift=1.5cm, minimum height=0.7cm]{Message Bus};

    \node (kubernetes) [draw, dotted, fit=(driver) (bus) (operator) (act), label=Kubernetes] {};

    \draw[latex-latex] (sensor) -- (driverscript);
    \draw[latex-latex] (gadget) -- (actscript);

    % \path (bus) -- (driversidecar) coordinate[midway] (aux);
    \draw[latex-latex] (bus.south -| driversidecar.north) -- (driversidecar);
    \draw[latex-latex] (bus.south -| ausidecar.north) -- (ausidecar);
    \draw[latex-latex] (bus.south -| actsidecar.north) -- (actsidecar);

    \draw[latex-latex] (operator.north -| driver.south) -- (driver);
    \draw[latex-latex] (operator.north -| au.south) -- (au);
    \draw[latex-latex] (operator.north -| act.south) -- (act);
\end{tikzpicture}

==> fever-screening-diagram.tex <==
\begin{tikzpicture}[node distance=0.4cm, auto, thick,scale=1, every node/.style={scale=0.75}]
    \node (camera) [sensor] {Visual Camera};
    \node (thermal) [sensor, below = of camera, yshift=-0.5cm] {Thermal Camera};
    \node (person) [au, right = of camera] {Person Detection};
    \node (face) [au, right = of person] {Face Recognition};
    \node (temporal) [au, right = of face, yshift=-1cm] {Temporal Fusion};
    \node (spatial) [au, right = of temporal] {Spatial Fusion};
    \node (fever) [au, right = of spatial] {Fever Screening};
    \node (gate) [gadget, right = of fever] {Gate Control};
    \node (db) [database, right = of face, xshift=2.2cm, yshift=1cm] {Registered Faces};

    \draw[->] (camera) -- (person);
    \draw[->] (person) -- (face);
    \draw[->] (face) -| (temporal);
    \draw[->] (thermal) -| (temporal);
    \draw[->] (temporal) -- (spatial);
    \draw[->] (spatial) -- (fever);
    \draw[->] (fever) -- (gate);
    \draw[<->] (face.north) |- (db);

\end{tikzpicture}


==> steps.tex <==
\begin{tikzpicture}[node distance=0.5cm, auto, thick,scale=1, every node/.style={scale=0.75}]
    \node (s1) [requiredstep] {Register drivers, AUs, and actuators};
    \node (s2) [optionalstep, right = of s1] {Create databases};
    \node (s3) [requiredstep, right = of s2] {Register sensors};
    \node (s4) [requiredstep, right = of s3] {Define autgmented streams using AUs};
    \node (s5) [optionalstep, right = of s4] {Register gradgets};
    \draw[->] (s1) -- (s2);
    \draw[->] (s2) -- (s3);
    \draw[->] (s3) -- (s4);
    \draw[->] (s4) -- (s5);
\end{tikzpicture}

